Emergence of complex network topologies from flow-weighted optimization of network efficiency

Transportation and distribution networks are a class of spatial networks that have been of interest in recent years. These networks are often characterized by the presence of complex structures such as central loops paired with peripheral branches, which can appear both in natural and man-made systems, such as subway and railway networks. In this study, we investigate the conditions for the emergence of these non-trivial topological structures in the context of human transportation in cities. We propose a minimal model for spatial networks generation, where a network lattice acts as a spatial substrate and edge velocities and distances define an effective temporal distance which quantifies the efficiency in exploring the urban space. Complex network topologies can be recovered from the optimization of joint network paths and we study how the interplay between a flow probability between two nodes in space and the associated travel cost influences the resulting optimal network. In the perspective of urban transportation we simulate these flows by means of human mobility models to obtain Origin-Destination matrices. We find that when using simple lattices, the obtained optimal topologies transition from tree-like structures to more regular networks, depending on the spatial range of flows. Remarkably, we find that branches paired to large loops structures appear as optimal structures when the network is optimized for an interplay between heterogeneous mobility patterns of small range travels and longer range ones typical of commuting. Finally, we show that our framework is able to recover the statistical spatial properties of the Greater London Area subway network.

==> [Main + SM] Emergence of complex network topologies from flow-weighted optimization of network efficiency/apssamp.tex <==

%%%%%
% add info
\setcounter{figure}{0}
\setcounter{equation}{0}
\setcounter{table}{0}
\setcounter{section}{0}

%\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\thesection}{S\arabic{section}}
\renewcommand{\thesubsection}{S\arabic{section}.\arabic{subsection}}
\renewcommand{\thetable}{S\arabic{table}}
\renewcommand{\theequation}{S\arabic{equation}}
%%%%%

\renewcommand{\figurename}{\textbf{Supplementary Figure S}}
\makeatletter
\def\fnum@figure{\figurename\thefigure}
\makeatother



\section*{Supplementary Material for ``Emergence of complex networks topologies from flow-weighted optimization of network efficiency"}





\section{\label{sec:simple_models} Application On Simple Network Substrates}



In this Section we report more detailed results for the optimization of simple network substrates that was discussed in the Main text, specifically for the triangular (HEX) lattice (planar dual of the hexagonal tiling of space) and Erd\H{o}s-Rényi (ER) network. The aim is to explore the resulting topologies that emerge both in spatial and non spatial networks when simple probabilities are taken into consideration (see Main text).


\subsection{HEX Lattice and ER Network}

Results of model application on the triangular (HEX) lattice and results of model application on an Erd\H{o}s-Rényi (ER) non-spatial network. For the non-spatial generative model, an ensemble of 20 networks with N = 30 nodes and edge probability $\rho = 0.2$ is generated. For the spatial case, the optimization process is repeated 20 times for each value of $\beta$ on the triangular lattice with N = 37 nodes.\\

SM Fig. 1 and SM Fig. 2 show boxplots for the distributions of metrics computed on the cycle basis in panels A on both figures. In panels B, samples of the optimized network states are shown for different values of $\beta$.


\begin{figure}[H]
    \centering
    \includegraphics[width=0.85\linewidth]{images/SM_Fig_HexSimple_COMPOSITE.pdf}
    \caption{
    \small{
        \textbf{Cycle basis properties and samples - HEX lattice.}
        Boxplot statistics for the cycle basis dimension and optimal network samples for triangular lattice across different $\beta$ values. 
    }
    }
    \label{fig:HexSimple_COMP}
\end{figure}


%\begin{figure}
%    \centering
%    \includegraphics[width=0.8\linewidth]{images/ER_beta_boxplot.png}
%    \caption{
%        \textbf{Cycle Basis properties - ER network}
%        Boxplot Statistics for the cycle basis dimension in an ER network of% 50 nodes with connection probability $\rho = 0.15$
%    }
%    \label{fig:pipeline_scheme}
%\end{figure}

%\begin{figure}
%    \centering
%    \includegraphics[width=1.0\linewidth]{images/SM_Fig_ERSimple.pdf}
%    \caption{
%        \textbf{Samples - ER lattice}
%        Optimal network samples for ER Networks across different $\beta$ 
%    }
%    \label{fig:pipeline_scheme}
%\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.85\linewidth]{images/SM_Fig_ERSimple_COMPOSITE.pdf}
    \caption{
    \small{
        \textbf{Cycle basis properties and samples - ER network.}
        Boxplot statistics for the cycle basis dimension and optimal network samples for an Erdos-Renyi (ER) network across different $\beta$ values.
    }
    }
    \label{fig:ERSimple_COMP}
\end{figure}

\newpage






\section{Leaves patterns}

Here we show an application of the model to reproduce leaf venation patterns \cite{Katifori2010}. A single attracting node (single target or sink) is considered at one of the perimeter nodes of the lattice, and the substrate is optimized using all the other nodes as sources.


\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{images/leaves_TMP.png}
    \caption{
        \textbf{Optimal networks resembling leaves' veins patterns.}
        Optimal state when a single target (orange node) in a single spatial extremity is considered. Efficiency is optimized for all nodes in space to reach the target. The resulting optimal state resembles tree-like patterns found in leaves (A), while the distribution of edges weights is shown in (B).
    }
    \label{fig:leaves}
\end{figure}





\newpage

\section{Application on London Tube network}

In this section we discuss more in detail the application of the model on the Greater London Area urban morphology. We show that the London subway network spatial properties can be recovered by means of the optimal network state.\\
In particular, to simulate a real transportation system, an upper bound on edges travel velocity is imposed.

%The model accepts $T_{ij}$ data so we simulate them to have a proper spatial resolution. Ultimately one might opt to work with real data

\subsection{Data Integration: Census and OpenStreetMap Data}

To extend the model to real urban scenarios, we gather data regarding the urban morphological structure from OpenStreetMap (OSM) \cite{OpenStreetMap} and Census.

\subsubsection{OSM Data}

To model the attractiveness of nodes in the lattice, we use the density of Points Of Interest in the urban space.
We use amenities \cite{Hidalgo_2020} points in OSM as a proxy for Points Of Interest (POIs), and a node $j$ attractiveness ($W_{j}$) therefore encodes the density of amenities in space.

The bounding box for Greater London Area (GLA) is obtained via OSM (\url{https://wiki.openstreetmap.org/wiki/Bounding_Box}) and POI densities are recovered inside this box. Specifically we use the following amenities sub-categories:

\begin{center}
    \texttt{'cafe','college','library','school','university','kindergarten','restaurant','pub',
    'fast food','bar','bank','dentist','pharmacy','hospital','clinic','doctor','arts centre','cinema','community centre','police','post office','marketplace'}
\end{center}

In Fig. S\ref{fig:OSM} the amenities points recovered from OSM are plotted in the bounding box.


\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{images/SM_Fig_OSM.pdf}
    \caption{
    \small{
        \textbf{OSM amenities query for GLA bounding box.}
        Amenities retrieved from OSM (\url{https://openstreetmap.org/copyright}) for the bounding box defined by the following longitude $\[-0.6,0.35 \]$ and latitude interval $\[51.25,51.75\]$.
    }}
    \label{fig:OSM}
\end{figure}


\subsubsection{Census Data}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{images/SM_Fig_census.pdf}
    \caption{
    \small{
        \textbf{Census data retrieval.}
        \textbf{A)} London's wards data from Census 2014 (\url{https://data.london.gov.uk/dataset/ward-profiles-and-atlas}). \textbf{B)} Points are generated in space following wards polygons with a density proportional to Census data. \textbf{C)} Points are mapped to HEX3 tiles with associated densities of points. Finally, a restriction to a disc is used to enforce symmetry in the distribution of nodes and to ease the computational load.
    }}
    \label{fig:census}
\end{figure}

Points are mapped to density in space by using HEX3 tiling (\url{https://eng.uber.com/h3/}) with spatial resolution $RES$ = 8. This spatial discretization process via tiling is of particular relevance to map this information to the HEX triangular lattice model which was described in the Main text. Both Fig. S\ref{fig:census} and Fig. S\ref{fig:OSM} show how model information $P_{i}$ and $W_{j}$ are recovered from data and then mapped to tiles as in shown in panel C in Fig. S\ref{fig:census}. Tiles covering the urban area are then mapped to the spatial network model as nodes in the triangular lattice (see Fig. 5 in Main text).\\


For computational simplicity and to preserve the isotropy of the lattice substrate from its central point, we restrict our analysis to a disc centered in the London's region with highest attractiveness, that lies approximately in the City Of London district. Results are robust against integration of the remaining GLA region. As the optimal edges weights are influenced by the traffic on the substrate, the discarded regions in the Greater London Area do not add relevant contributions when compared to more central regions with higher population density.

%\subsection{Check of real OD matrices VS Spatial interaction model}
%\seba{Add figure with OD simulated compared to real OD for LGA, or simply the distribution of %trips probabilities}



\subsection{Results with distributions for traffic and bounded weights distribution}

To simulate a real system we limit upper edges weights to a fixed value $w^{*} = 7*w_{init}$ where $w_{init}$ is the initial edges weight assigned to the network state ($w_{init} = 1.0$) before optimization process, such that $\sum_{e \in G} d_{e} w_{e, init} = C$. In this simulation we work with $\beta = 0.35$. 

%We also show that the statistical properties are robust against a range of values for beta, as the traffic remains biased towards the same regions. It should probably instead be fitted from real OD data.
%Here we plot traffic distributions coming from the spatial interaction model, paired with the weight distribution of the optimized network state


\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{images/SM_Fig_LGAModel.pdf}
    \caption{
    \small{
        \textbf{Mapping the data to Hex lattice + GLA optimized network.}
    \textbf{A)} Urban morphology data mapped to the HEX tiling and then mapped to the triangular (HEX) lattice. At this step, OD matrix is generated and the network is then optimized. \textbf{B)} Resulting optimal network state with its distribution of edges weights showing a bi-modal shape. Only fast edges having weight larger than a threshold ($w_{e} > 5$) are kept to isolate the sub-graph constituted by a high velocity set of edges, such as a subway system.
    }}
    \label{fig:hex_mapping}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{images/SM_Fig_LGADiscrete.pdf}
    \caption{
    \small{
        \textbf{Pruned network vs real tube.}
    \textbf{A)} London subway network, restricted to the disc under study. \textbf{B)} GLA model output, limited to the nodes and edges which have a weight $w_{e} > 5.0$, where this value was chosen from the previously plotted $\{w_{e}\}$ distribution as a threshold to separate the second ``mode" with fast edges. This ``discretized" network is the model on which statistical measures are performed.
    }}
    \label{fig:pruned_network}
\end{figure}


\newpage


\section{Scaling of network stations}

The spatial organization of the transportation network can be inspected by taking into consideration the number of nodes' stations $N(r)$ up to a distance $r$ from the barycenter of stations. In the Main text we analyze the scaling regimes for the simulated and real London Tube network \cite{Gallotti2015} following the analysis employed in \cite{Roth2012}. Specifically, they obtain functional forms for the scaling properties of $N(r)$ for different distances from the barycenter. We report here the scalings obtained in \cite{Roth2012}:

\begin{equation}
    N(r) \sim \begin{cases}\rho_C \pi r^2 & \text { for } r<r_C \\ \rho_C \pi r_C^2+\mathcal{N}_B \int_{r_C}^r \frac{d r}{\Delta(r)} & \text { for } \quad r_C<r<r_{\max } \\ N & \text { for } r>r_{\max }\end{cases}
    \label{eq:scalings}
\end{equation}

Specifically, they show that in the large distance regime ($r > r_{C}$ and $r < r_{\max}$ ) the number of stations can be approximated by adding the integral curve $\mathcal{N}_B \int_{r_C}^r \frac{d r}{\Delta(r)}$ to a constant term. In \cite{Roth2012} it is also reported that the large distance behavior can be also, in general, approximated by a scaling law. 
Therefore we plot here the computation of the integral curve against rescaled values of $r$, and show that in that regime it can be approximated by a power law, and its exponent can be obtained via a linear fit. The $N(r)$ curve in the Main text was computed on the real London Tube restricted to the disc area as presented in SM Fig. \ref{fig:pruned_network}.
The associated exponent $\gamma = 1.25 \pm 0.02$ was used in the Main text to highlight the secondary scaling for $r > r_{C}$. As discussed in Ref. \cite{Roth2012}, due to $\Delta(r)$ in SM Eq. \ref{eq:scalings} being often noisy, this scaling property is not often well reproduced in empirical networks, and it is often restricted to a small region of $r$ values. In Fig. 6 of the Main text, we see that the secondary scaling with the exponent $\gamma$ approximates $N(r)$ in a limited interval for $r > r_{C}$. The value of the exponent in the branches region is expected to be $\gamma < 2.0$ \cite{Roth2012} and our result is consistent with this.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{images/scaling_gamma.png}
    \caption{
    \small{
        \textbf{Scaling of the integral curve.}
        Log-Log plot of the integral curve and its linear fit. With the associated value of the $\gamma$ exponent approximated, to highlight a secondary scaling region as mentioned in \cite{Roth2012}.
    }}
    \label{fig:scaling-integral}
\end{figure}


\clearpage
%\nocite{*}
\bibliography{apssamp}% Produces the bibliography via BibTeX.

\end{document}
%
% ****** End of file apssamp.tex ******

